Temporal Robustness of Temporal Logic Specifications: Analysis and Control Design

We study the temporal robustness of temporal logic specifications and show how to design temporally robust control laws for time-critical control systems. This topic is of particular interest in connected systems and interleaving processes such as multi-robot and human-robot systems where uncertainty in the behavior of individual agents and humans can induce timing uncertainty. Despite the importance of time-critical systems, temporal robustness of temporal logic specifications has not been studied, especially from a control design point of view. We define synchronous and asynchronous temporal robustness and show that these notions quantify the robustness with respect to synchronous and asynchronous time shifts in the predicates of the temporal logic specification. It is further shown that the synchronous temporal robustness upper bounds the asynchronous temporal robustness. We then study the control design problem in which we aim to design a control law that maximizes the temporal robustness of a dynamical system. Our solution consists of a Mixed-Integer Linear Programming (MILP) encoding that can be used to obtain a sequence of optimal control inputs. While asynchronous temporal robustness is arguably more nuanced than synchronous temporal robustness, we show that control design using synchronous temporal robustness is computationally more efficient. This trade-off can be exploited by the designer depending on the particular application at hand. We conclude the paper with a variety of case studies.

==> chapters/2del/dynamics.tex <==
\section{UAS dynamics}
\label{sec:dynamics}

\todo{Do we ignore constraints on the
	UAS inputs? The equation~\eqref{eq:dyn_inp}}
\todo{Change xyz axis to capital, but state to just x? Rest of the paper uses x for the state.}

\begin{figure}[h!]
	\centering
	\includegraphics[width=.5\textwidth]{figures/frames.png}
	\caption{Internal world frame with rotation angles $\eta$ (left) and UAS body frame
with angular rates $\omega$ (right). Gravity is denoted as $\mathbf{g}$,
	thrust force $f$ pointing along the axis $e_3$.
		 Figure adapted from \cite{mueller2015computationally}.}
	\label{fig:frames}
\end{figure}

Multi-rotor dynamics have been studied extensively in the
literature \cite{luukkonen2011modelling}, \cite{mueller2015computationally}, and we closely follow the conventions of
\cite{mueller2015computationally}. %Fig. 9 illustrates the following definitions. 

The UAS is modeled as a rigid body with 6
degrees of freedom. The first three are 
the absolute linear position of the UAS in the orthogonal inertial frame, $p = [x, y, z]^\top\in\mathbb{R}^3$. 
The remaining
three are the rotation angles $\eta=[\phi, \theta, \psi]^\top\in\mathbb{R}^3$ that correspond to roll, pitch and yaw, respectfully, of the UAS body
frame with respect to the internal world frame. Rotation at time $t$ is defined by the rotation
matrix $\mathbf{R}\in\mathbb{R}^{3\times3}$, see \cite{luukkonen2011modelling} for the exact expression.
The corresponding time-derivatives of $\eta$ define UAS' angular velocities, $\omega=[\omega_1, \omega_2, \omega_3]^\top$. 

%We write $v = \dot{p}$ for linear velocity and $a 
%=\dot{v}$ for acceleration. 

Let $m$ be the mass of the UAS, $\mathbf{g}=[0,0,-g]^\top$ the acceleration due to gravity and $e_3 = [0, 0, 1]^\top$ a constant vector in the UAS body frame corresponding the thrust force axis\footnote{UAS' thrust direction in the internal world frame is $\mathbf{R}e_3$}, see Figure~\ref{fig:frames}, then
the dynamics is given by
\begin{equation}
\label{eq:dyn}
m\ddot{p} = \mathbf{R}e_3 f + m\mathbf{g}
\end{equation}

\begin{equation}
\label{eq:dyn_inp}
\dot{\mathbf{R}} = \mathbf{R} 
\begin{bmatrix}
0 & -\omega_3 & \omega_2 \\
\omega_3 & 0 & \omega_1\\
-\omega_2 & \omega_1 & 0
\end{bmatrix}
\end{equation}

By substituting matrix $\mathbf{R}$ from \cite{luukkonen2011modelling} in equation~\eqref{eq:dyn}  we obtain the following equation:
\begin{equation}
m\begin{bmatrix}
\ddot{x} \\\ddot{y} \\\ddot{z}
\end{bmatrix}=
\begin{bmatrix}
\cos\psi\sin\theta \cos\phi +\sin\psi\sin\phi \\
\sin\psi\sin\theta\cos\phi - \cos\psi\sin\phi\\
\cos\theta\cos\phi
\end{bmatrix} f - m
\begin{bmatrix}
0 \\ 0\\g
\end{bmatrix}
\end{equation}

With an assumption of no yaw motion (fixed $\psi=0$) we get the following dynamic system: 
\begin{equation}
\label{eq:dyn_simp}
\begin{bmatrix}
\ddot{x} \\\ddot{y} \\\ddot{z}
\end{bmatrix}=
\frac{1}{m}
\begin{bmatrix}
\sin\theta \cos\phi\\
- \sin\phi\\
\cos\theta\cos\phi
\end{bmatrix} f - 
\begin{bmatrix}
0 \\ 0\\g
\end{bmatrix}
\end{equation}

Let the control inputs be roll, pitch and thrust of the UAS, therefore,
$\mathbf{u}=[\phi, \theta, f]^\top\in\mathbb{R}^3$. Denote the full UAS' state as $\mathbf{x}=[x,y,z,\dot{x}, \dot{y},\dot{z}]^\top=[p, v]^\top\in\mathbb{R}^6$. Equation \eqref{eq:dyn_simp} can be written as
\begin{equation}
\label{eq:dyn_general}
\dot{\mathbf{x}} = f(\mathbf{x}, \mathbf{u}).
\end{equation}
The linearization of \eqref{eq:dyn_simp} around hover $\bar{\mathbf{u}}=(0, 0, mg)$ leads to the following system: 
\begin{equation}
\dot{\mathbf{x}} = \left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d \mathbf{x}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} \mathbf{x} +
\left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d\mathbf{u}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} \mathbf{u}
\end{equation}
In other words, we can rewrite \eqref{eq:dyn_general} as the following Linear Time-Invariant (LTI) ODE:
\begin{equation}
\label{eq:dyn_cont}
\dot{\mathbf{x}}(t) = A_c \mathbf{x}(t) + B_c \mathbf{u}(t)
\end{equation}
where 
\begin{equation}
A_c = \left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d\mathbf{x}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} = \begin{bmatrix}
\mathbf{0}_{3\times3} & I_{3\times 3} \\
\mathbf{0}_{3\times3} & \mathbf{0}_{3\times3}
\end{bmatrix},
\end{equation}
\begin{equation}
B_c = \left.\frac{\partial f(\mathbf{x}, \mathbf{u})}{d\mathbf{u}}\right\vert_{\substack{\mathbf{x}=\bar{\mathbf{x}}\\ \mathbf{u}=\bar{\mathbf{u}}}} = \begin{bmatrix}
&\mathbf{0}_{3\times 3}&\\
0 & g & 0\\
-g & 0 & 0 \\
0 & 0 & \frac{1}{m}
\end{bmatrix}.
\end{equation}
Therefore, the UAS dynamics can be described as following: 
\begin{equation}
\label{eq:dyn_simp2}
\begin{bmatrix}
	\ddot{x} \\\ddot{y} \\\ddot{z}
\end{bmatrix}=
\begin{bmatrix}
	g\theta\\
	- g\phi\\
	\frac{1}{m} f
\end{bmatrix} 
\end{equation}
Discretization of equation~\eqref{eq:dyn_cont} following \cite{pant2015co} leads to:
\begin{equation}
\label{eq:dyn_k}
\mathbf{x}_{k+1}= A \mathbf{x}_k + B \mathbf{u}_k.
\end{equation}

The preceding model \eqref{eq:dyn_simp2} is a simplification of complex dynamic interactions.
There exist other more sophisticated UAS models. For example, dynamic model in \cite{bouadi2007nonlinear} includes drag force generated by the air resistance. 
Models studied in \cite{hoffmann2007quadrotor} and \cite{huang2009aerodynamics} include 
dependence of thrust on angle of attack, blade flapping and airflow disruptions.
The influence of aerodynamical effects is complicated
and some of the effects have significant impact
only in high velocities and regimes beyond nominal hover conditions. 
Thus, these effects are excluded from the model used in this paper.
The dynamic model \eqref{eq:dyn_simp2} captures the most relevant dynamics and yields tractable solutions to the trajectory generation problem.
Furthermore, in many applications, for
example, model predictive control, such a simple model is
sufficient, with continuous replanning compensating for modeling inaccuracies.



==> chapters/2del/space_time_comparison.tex <==
 
\subsection{Space-robustness perspective}
Denote $\mathcal{L}(\varphi)=\{t\in\TDom\ |\ \chi_\varphi(\sstraj, t)=+1\}$ (why trajectory is restricted?)


$\Dist{t}^+(\sstraj(t), \mathcal{L}(\varphi))$

==> chapters/2del/sup_sync.tex <==
\newpage

	Donze's definition:
	\begin{equation}
		\thetap_p(\sstraj,t) = \chi_p(\sstraj, t)\cdot
		\max\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau],\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)\}
	\end{equation}
The work with continuous trajs of $\TDom=\Re_{\geq 0}$, so unbounded.
But it is not formally correct. I assume the $\max$ should be $\sup$.

Take a look at Fig.~\ref{fig:draft_sup}. 
\begin{figure}[h!]
	\centering
	\includegraphics[width=.6\textwidth]{chapters/2del/figures/draft_sup.jpg}
	\caption{Example.}
	\label{fig:draft_sup}
	\vspace{-5mm}
\end{figure}
\begin{itemize}
	\item In sub-figure (a) we get $\thetap_p(\sstraj,0)=\pi$. 
	\item In (b) $\thetap_p(\sstraj,0)=0$ since $\chi_p(\sstraj,0)=+1\not= -1 =\chi_p(\sstraj,\epsilon)$.
	\item In (b) $\thetap_p(\sstraj,\frac{\pi}{2})=\frac{\pi}{2}$ though $\chi_p(\sstraj,\frac{\pi}{2})=-1\not=\chi_p(\sstraj,\pi)=+1$.
\end{itemize}

1. Should it then be $[t, t+\tau)$ instead of $[t,t+\tau]$? Do we get the same result if we have closed or half-open anyway, since we use $\sup$?

2. We mush work with $\theta\in\CoRe$ because $\tau=+\infty$ is a possibility ($\TDom$ can still be $\Re$). So we need supremum of unbounded set, if we are on $\Re$ it is undefined. For this case it could be half open or closed, does not matter. If we had $\TDom=\CoRe_{\geq 0}=\Re_{\geq 0}\cup\{+\infty\}$ we can say both $[t,t+\infty]$ and $[t,t+\infty)$. Intersect $t'$ with $\TDom$:
	\begin{equation}
	\thetap_p(\sstraj,t) = \chi_p(\sstraj, t)\cdot
	\sup\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau)\cap\TDom,\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)\}
\end{equation}
But then if $\TDom=[0,H]]$ we need to bound $\tau$ too, no? otherwise $\tau=100500$ works because $[0, 100500)\cap [0, H]=[0, H]$.

3. If the interval is half-open then we DO NOT need to define $\theta=0$ as a separate case because
\begin{align*}
	&\sup\{\tau\geq0 \ :\ \forall t'\in [t,t+\tau),\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)\}= \\
	&\sup\{\tau\geq0 \ :\ \forall t'\in\emptyset,\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)\}=\\ 
	&\sup\{\tau\geq0 \ :\ \forall t'\ [t'\in\emptyset\Longrightarrow\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)]\}=\\
	&\sup\{\tau\geq0 \ :\ \forall t'\ [\bot \Longrightarrow\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)]\}=\\
	&\sup\{\tau\geq0 \ :\ \forall t'.\ \top\}
\end{align*}

4. Then all theorems would state smth like for all $t'\in t+[0, i)$ property holds. So $t+i$ should be excluded. Same as the open ball for space domain. 

5. Let's consider a simple case when $\chi_p(\sstraj,0)=+1$, then 
\begin{equation*}
	\thetap_p(\sstraj,0) = 
	\sup\{\tau\geq0 \ :\ \forall t'\in[0,\tau),\ \chi_p(\sstraj,t')=+1\}= 1.
\end{equation*}
It follows that $\forall t\in [0, 1)$, $\chi_p(\sstraj,t)=+1$. But what else does it mean from iff point of view? For example for a discrete case, $\theta=1$ iff $\forall t\in [0, 1)$, $\chi_p(\sstraj,t)=+1$ and $\chi_p(\sstraj,1)=-1$.
How to do smth similar in cont case? 
I think the following holds: $\theta_p(\sstraj,t)=i$ iff
\begin{align*}
&\forall t'\in [t, t+i), \chi_p(\sstraj,t')=\chi_p(\sstraj,t) \\
&\text{and}\quad (\chi_p(\sstraj,t+i)\not=\chi_p(\sstraj,t)\quad\text{or}\quad\exists \epsilon> 0,\ \forall t''\in (t+i,t+i+\epsilon].\ \chi_p(\sstraj,t'')\not=\chi_p(\sstraj,t)) 	
\end{align*}

\underline{Here is logic why it works:}
Consider $\chi=+1$ on $A=[0,1]$ and on $A=[0, 1)$ and $-1$ otherwise, see Fig.~\ref{fig:draft_sup2}. 
\begin{figure}[h!]
	\centering
	\includegraphics[width=.6\textwidth]{chapters/2del/figures/draft_sup2.jpg}
	\caption{Example.}
	\label{fig:draft_sup2}
	\vspace{-5mm}
\end{figure}
In both cases, the $\theta(0)=\sup A = 1$. 
In both cases same as before we know that for sure $\forall t\in [0,1), \chi=+1$. But at 1 itself the result will differ based on the case: $\chi(1)=+1$ in the first case; $\chi(1)=-1$ in the second case (In first case, $1\in A$; in the second one $1\not\in A$).
So in the first case, $\exists \epsilon>0$ s.t. $\chi(1+\epsilon)=-1$. In the second case $\chi(1)=-1$. 

6. How to show that 	
\begin{align*}
	&\sup\{\tau\geq0 \ :\ \forall t\in[0,\tau),\ \chi_{p_1}(\sstraj,t)=+1\}=i_1>0\\
	&\sup\{\tau\geq0 \ :\ \forall t\in[0,\tau),\ \chi_{p_2}(\sstraj,t)=+1\}=i_2 \geq i_1
\end{align*}
leads to
\begin{align*}
	&\sup\{\tau\geq0 \ :\ \forall t\in[0,\tau),\ \chi_{p_1 \wedge p_2}(\sstraj,t)=+1\}=i_1
\end{align*}
\begin{proof}
	Denote $S_k=\{\tau\geq0 \ :\ \forall t\in[0,\tau),\ \chi_{p_k}(\sstraj,t)=+1\}$.
	
	By definition $\sup S_k = i_k$ 
	iff 
	
	(1) $\forall x\in S_k$, $x\leq i_k$ and 
	
	(2) $\forall \alpha_k$ such that $\forall x\in S_k$, $x\leq \alpha_k$ it holds that $i_k\leq \alpha_k$.
	
	Now consider 
	\begin{align*}
		S = &\{\tau\geq0 \ :\ \forall t\in[0,\tau),\ \chi_{p_1 \wedge p_2}(\sstraj,t)=+1\}=\\
		&\{\tau\geq0 \ :\ \forall t\in[0,\tau),\ \chi_{p_1}(\sstraj,t)=+1 \wedge \chi_{p_2}(\sstraj,t)=+1\}=\\
		&S_1 \cap S_2.
	\end{align*}
Let's see if the properties required for $\sup S=i_1$ hold. 

1. $\forall x\in S= S_1 \cap S_2$ we get $x\in S_1$ and $x\in S_2$. 
	Since $x\in S_1$ then $x\leq i_1$. Since $x\in S_2$ we get $x\leq i_2$ where $i_2\geq i_1$. Therefore, $x\leq \min(i_1,i_2)=i_1$. Holds.
	
2. Take any $\alpha$ such that $\forall x\in S$, $x\leq \alpha$.
Since $x\in S$ it means $x\in S_1$. Since $x\in S_1$ and $x\leq \alpha$ then $i_1\leq \alpha$.
	
	-----------------------------------------------------------------------------
	
TO SUMMARIZE EVERYTHING:
For $\TDom \subseteq \Re$, $\theta^{\pm}_\varphi\in \CoRe$ is defined recursively:
	\begin{equation}
	\thetap_p(\sstraj,t) = \chi_p(\sstraj, t)\cdot
	\sup\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_p(\sstraj,t')=\chi_p(\sstraj,t)\}
\end{equation}




%	\begin{lemma}
%		Suppose $A_i \subseteq\Re$, $i=1,\ldots,n$ are nonempty subsets of $\Re$ such that $\bigcap A_i \not=\emptyset$.
%		Then 
%		\begin{equation}
%			\sup \bigcap_{i=1}^n A_i = \bigsqcap_{i=1}^n \sup A_i
%		\end{equation}
%		\end{lemma}
%	\begin{proof}
%		First, remember that if $A\subseteq B \subseteq\Re$, $A\not=\emptyset$ and $B$ is bounded above then $\sup A \leq \sup B$. Easy to see that the same fact holds for $A\subseteq B \subseteq\CoRe$ without constraints on empty/boundedness ($\sup\emptyset =-\infty < +\infty=\sup \CoRe)$.
%		
%		Therefore, since $\bigcap_{i=1}^n A_i \subset A_i$, therefore, $\sup \bigcap_{i=1}^n A_i \leq \sup A_i$, for all $i$. Since it holds for all $i$, then  $\sup \bigcap_{i=1}^n A_i \leq \bigsqcap_{i=1}^n \sup A_i$.
%		
%		Since $\bigcap A_i \not=\emptyset$ then if $x\in \bigcap A_i$, then $x\in A_i$ for all $i$. And therefore, $x\leq \sup A_i$.
%	
%	\end{proof}
%	Now
%	let $A_i=\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_i}(\sstraj,t')=+1\}\subseteq\Re$, where $i=\{1,2\}$. Each and their intersection is not empty (at least $\tau=0$ belongs to them all. Then using the lemma above, 
%	\begin{align*}
%		&\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_1 \wedge \varphi_2}(\sstraj,t')=+1\}=\\
%		&\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_1}(\sstraj,t')\sqcap \chi_{\varphi_2}(\sstraj,t')=+1\}=\\
%		&\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_1}(\sstraj,t')=+1 \wedge\chi_{\varphi_2}(\sstraj,t')=+1\}\overset{\color{red}\text{R U sure???}}{=}\\
%		&\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_1}(\sstraj,t')=+1\} \cap
%		\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_2}(\sstraj,t')=+1\}=\\
%		&A_1 \cap A_2.
%	\end{align*}
%Therefore, $\sup\{\tau\geq0 \ :\ \forall t'\in[t,t+\tau),\ \chi_{\varphi_1 \wedge \varphi_2}(\sstraj,t')=+1\} = \sup (A_1\cap A_2)= \min( \sup A_1,\ \sup A_2)= \min(i,j)=i$.
\end{proof}
\newpage

==> chapters/extra_lemmas.tex <==
\section{Extra lemmas}



\begin{rem}
	Note that our definition of asynchronous temporal robustness \ref{def:time_rob_rec} is a modified temporal robustness definition from \cite{Donze10STLRob}.
	%$$\thetap_p(\sstraj, t)= \chi_\varphi(\sstraj, t) \cdot
	%\max\{ \tau\geq 0,\ \forall t'\in [t, t+\tau],\ \chi_\varphi(\sstraj,t')=\chi_p(\varphi,t)\}$$
	Our version is properly defined because we fix the following issues that \cite{Donze10STLRob} has:
	\begin{enumerate}
		\item Authors in \cite{Donze10STLRob} use $\max$ operator. If signal never changes its satisfaction in the future then $\max$ is undefined. We fix this issue by using $\sup$ operator together with setting the temporal robustness domain to be the extended real line $\CoRe$ to account for the cases when temporal robustness equals to $\pm \infty$. 
		\item $\max$ operator also struggles with cases when satisfaction does not change on the right-open intervals, for example, when $\chi_p(\sstraj,t')=+1$ for $\forall t'\in[t, t+10)$ and $\chi_p(\sstraj,t+10)=-1$. In this case, $\max$ is undefined. Our $\sup$ definition is properly defined and leads to time $\thetap_p(\sstraj, t)= 10$.
		\item  Authors in \cite{Donze10STLRob} use $\chi_\varphi(\sstraj,t')$ in the definition of temporal robustness for a predicate $p$ which we assume is a typo since they advocate for the inductive definition. We use corrected $\chi_p(\sstraj,t')$.
		Authors in \cite{Donze10STLRob} also only refer to recursive rules for negation and conjunction without defining the temporal robustness for the Until operator. We use the full STL semantics. 
		\item Authors in \cite{Donze10STLRob} state a single theorem on the connection between the temporal robustness value and the amount of shifts allowed where authors refer to `shifting events' though never properly define neither the event nor the synchronous or asynchronous nature of such shifts. Also, the proof is missing. We present all proofs for theorems we use in our paper.
	\end{enumerate} 
\end{rem}

The following remark directly follows from Thm.~\ref{thm:sat_eta} and \ref{thm:sat_theta}:
	\begin{rem}
		\label{rem:abs}
		\begin{enumerate} For an STL formula $\varphi$, signal $\sstraj:\TDom \rightarrow X$, time $t\in\TDom$ the following results hold:
			\item\label{extra:eta} $\eta^{\pm}_\varphi(\sstraj,t) = \chi_\varphi(\sstraj,t) \cdot |\eta^{\pm}_\varphi(\sstraj,t)|$.
			\item\label{extra:theta} $\theta^{\pm}_\varphi(\sstraj,t) = \chi_\varphi(\sstraj,t) \cdot |\theta^{\pm}_\varphi(\sstraj,t)|$.
		\end{enumerate}
	\end{rem}
	\begin{proof}
		Let $\zeta \in \{\eta^{\pm}_\varphi, \theta^{\pm}_\varphi\}$. 
		
		If $\zeta(\sstraj,t) >0$ then $\chi_\varphi(\sstraj,t)=+1$ and thus, $\eta^{\pm}_\varphi(\sstraj,t) = |\zeta(\sstraj,t)|$.
			
			If $\zeta(\sstraj,t) <0$ then $\chi_\varphi(\sstraj,t)=-1$ and thus, $\zeta(\sstraj,t) = -|\zeta(\sstraj,t)|$.
			
			If $\zeta(\sstraj,t) =0$ then $\zeta(\sstraj,t) =0= |\zeta(\sstraj,t)|$.
	\end{proof}

\begin{lemma}
	\label{lemma:sum} 
	For an STL formula $\varphi$, signal $\sstraj:\TDom \rightarrow X$, time $t\in\TDom$ and some value $i\in\CoRe_{\geq 0}$, the following results hold:
	\begin{enumerate}	
			\item $|\etap_\varphi(\sstraj, t) + \etam_\varphi(\sstraj, t)| = |\mathcal{T}_t|$, $\forall t\in \mathcal{T}_t$, where 
			
			$\mathcal{T}_t = \{\tau\ |\ \chi_\varphi(\sstraj,\tau)=\chi_\varphi(\sstraj,t)\ \wedge\ \mathcal{T}_t\,\text{is connected}\ \wedge\ t\in\mathcal{T}_t\}$
			
			in other words, $\etap_\varphi(\sstraj, t) + \etam_\varphi(\sstraj, t)$ is constant inside an interval in which the truth value of $\varphi$ is uniform and is equal to the length of this interval.
		{\color{red}
			\item NOT SURE THIS HOLDS:
			$|\thetap_\varphi(\sstraj, t) + \thetam_\varphi(\sstraj, t)| \leq |\mathcal{T}_t|$, $\forall t\in \mathcal{T}_t$, where 
			$\mathcal{T}_t = \{\tau\ |\ \chi_\varphi(\sstraj,\tau)=\chi_\varphi(\sstraj,t)\ \wedge\ \mathcal{T}_t\,\text{is connected}\ \wedge\ t\in\mathcal{T}_t\}$
			
			in other words, $\thetap_\varphi(\sstraj, t) + \thetam_\varphi(\sstraj, t)$ might not be a constant inside an interval in which the truth value of $\varphi$ is uniform but is bounded by its length.
		}	
	\end{enumerate}
\end{lemma}
{\color{red}
\begin{proof}
		\begin{enumerate}
				\item Take any $t\in \TDom$ and determine $\mathcal{T}_t$. We know that $\forall \tau\in\mathcal{T}_t$, $\chi_\varphi(\sstraj,\tau)=\chi_\varphi(\sstraj,t)$.
				Assume that $\chi_\varphi(\sstraj, t)=+1$ then $\eta^{\pm}_\varphi(\sstraj, t) \geq 0$.
				Let $|\etap_\varphi(\sstraj, t)|=\etap_\varphi(\sstraj, t)= i\geq 0$ and 
				$|\etam_\varphi(\sstraj, t)|=\etam_\varphi(\sstraj, t)= j\geq 0$. Then according to Thm.~\ref{thm:chi_sync_stronger}, 
				$\forall h\in (-j, i),\ \chi_{\varphi}(\sstraj,t+ h)=\chi_\varphi(\sstraj,t)$. Also,  
				$\forall\epsilon>0$, $\exists \tilde{h}^+\in[i, i+\epsilon)$ and $\exists \tilde{h}^-\in[j, j+\epsilon)$ such that $\chi_{\varphi}(\sstraj,t - \tilde{h}^-)=\chi_{\varphi}(\sstraj,t + \tilde{h}^+)\not=\chi_\varphi(\sstraj,t)$.
				Thus, $|\mathcal{T}_t|=i+j$.
				For any $\tau\in\mathcal{T}$, ??
		\item Figure out the proof. 		
		\end{enumerate}		
\end{proof}
}

\begin{lemma}
	If $\mathbf{s}=\sstraj^{\leftrightarrows h}$ it \textbf{does not} follow that $s(t)=x(t \pm h)$. 
\end{lemma}
\begin{proof}
	First counter-example is: let $\mu(x_t)= x_t \geq 0$ and let $s(t)=ax(t+h)$, where $a>0$, i.e. $\mathbf{s}$ is a scaled and shifted $\sstraj$. Therefore, it does not hold that $s(t)=x(t \pm h)$ but it is also easy to see that  $\mathbf{s}=\sstraj^{\leftarrow h}$ since $\chi_p(s, t)= \sign(\mu(s_t)) = \sign( s_t \geq 0) = \sign( ax_{t+h} \geq 0)=\sign( x_{t+h} \geq 0)=\chi_p(x, t+h)$. 
	
	{\color{blue}
	Even if only shifts are allowed to obtain $\mathbf{s}$ and only linear predicates are used then
	$\chi_p(s, t)= \sign(\mu(s_t)) = \sign(a^\top s_t +b \geq 0)= \sign( a^\top (x^1_{t+h_1}; ...;x^n_{t+h_n}) + b \geq 0)= 1=\sign( a^\top x_{t+h} + b \geq 0)=\chi_p(x, t+h)$ if $a_i, x_t^i \geq 0$ and $b=0$, i.e. $\mathbf{s}=\sstraj^{\leftarrow h}$ and $s(t)\not=x(t \pm h)$ for any $h\not=\bar{h}$.
}
\end{proof}

==> chapters/lemmas.tex <==
\section{Laws of Quantifier Distribution}
%\begin{lemma}[The Order of Mixed Quantifiers]
%	\label{lemma:quant}
%	\begin{align*}
%		\exists x \forall y\  Q(x,y) \Longrightarrow \forall y \exists x\  Q(x,y)
%		%\\
%	%	\forall x \exists y\  Q(x,y)\  \not\!\!\Longrightarrow \exists y \forall x\  Q(x,y).
%	\end{align*}
%\end{lemma}	
%\begin{proof}
%	If there is a fixed $x^*$ which makes $Q(x,y)$
%	true for all $y$, then no matter what $y$ we are given, we can find a $x$ (the fixed value $x^*$) which makes $Q(x,y)$ true.
%	
%%	The fact that the second implication does not hold can be shown by a counterexample:
%%	$\forall x\exists y (x<y)$ is true and states that given any number there is a strictly larger number, that is, there is no largest number. The second sentence, $\exists y \forall x (x<y)$ is false. It says that there is a single number that is strictly larger than all real numbers, which is of course, false.
%\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}[Existential quantification over a set]
	\label{def:ex}
	\begin{equation*}
	\exists x\in X.\ P(x)\  \overset{\text{Def}}{\Longleftrightarrow}\  \exists x(x\in X\ \wedge\ P(x))
	\end{equation*}
\end{definition}

\begin{definition}[Universal quantification over a set]
	\label{def:uni}
	\begin{equation*}
	\forall y\in Y.\ P(y) \ \  \overset{\text{Def}}{\Longleftrightarrow}\ \forall y(y\in Y\ \Longrightarrow\ P(y))
	\end{equation*}
\end{definition}


\begin{lemma}[Quantifier Laws \cite{hammond2007introduction}]
\label{lemma:quant_laws}
	The following quantifier laws hold:
\begin{enumerate}
	\item\label{i:quant_scope}
	$\forall x \forall y\  P(x,y)\  \Longleftrightarrow\ \forall y \forall x P(x,y)$.
	%
	\item\label{i:quant}
	$	\exists x \forall y\  Q(x,y)\ \Longrightarrow\ \forall y \exists x\  Q(x,y)$.
	%
	\item\label{i:forall_exists}
	$\forall x P(x) \wedge \forall x Q(x)\  \Longleftrightarrow\ \forall x (P(x) \wedge Q(x))$.
	%
	\item\label{i:forall}
	$\forall x P(x) \vee \forall x Q(x)\ \, \Longrightarrow\ \,\forall x (P(x) \vee Q(x))$.
\end{enumerate}
\end{lemma}

%\begin{lemma}[Distribution of Quantifiers
%	over Disjunction \cite{hammond2007introduction}]
%	\label{lemma:forall}
%	\begin{align*}
%		\forall x P(x) \vee \forall x Q(x)\  \Longrightarrow&\ \forall x (P(x) \vee Q(x)).
%		%		\\\exists x (P(x) \vee Q(x))\ \Longleftrightarrow&\ \exists x P(x) \vee \exists x Q(x)
%	\end{align*}
%\end{lemma}	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma}[Laws of Quantifier Distribution: Equivalences \cite{hammond2007introduction}]
%	\label{lemma:forall_exists}
%	\begin{align*}
%		\forall x P(x) \wedge \forall x Q(x)\  \Longleftrightarrow&\ \forall x (P(x) \wedge Q(x))\\
%		\exists x P(x) \vee \exists x Q(x)\  \Longleftrightarrow&\ \exists x (P(x) \vee Q(x)).
%	\end{align*}
%\end{lemma}	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma}[Laws of Quantifier Scope \cite{hammond2007introduction}]
%	\label{lemma:quant_scope}
%	\begin{align*}
%		\forall x \forall y P(x,y)\  \Longleftrightarrow\ \forall y \forall x P(x,y).
%	\end{align*}
%\end{lemma}	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Quantifier Laws over Sets]
	\label{lemma:quant_laws_set}
	The following quantifier laws hold:
	\begin{enumerate}
		\item\label{i:quant_scope_set}
		$\forall x\in X,\ \forall y\in Y.\ P(x,y)\  \Longleftrightarrow\ 
		\forall y\in Y,\ \forall x\in X.\  P(x,y)$.
		%
		\item\label{i:quant_set}
		$	\exists x\in X,\ \forall y\in Y.\  Q(x,y)\ \Longrightarrow\ 
		\forall y\in Y,\ \exists x\in X.\  Q(x,y)$.
		%
		\item\label{i:forall_exists_set}
		$\forall x\in X.\ P(x) \ \wedge\ \forall x\in X.\ Q(x)\  \Longleftrightarrow\ 
		\forall x\in X\ (P(x) \wedge Q(x))$.
		%
		\item\label{i:forall_set}
		$\forall x\in X.\ P(x) \ \vee\ \forall x\in X.\ Q(x)\ \, \Longrightarrow\ \,\forall x\in X\  (P(x) \vee Q(x))$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	\begin{enumerate}
		\item The following sequence holds:
		\begin{align*}
			\forall x\in X,\ \forall y\in Y.\  P(x,y) &\overset{\ref{def:uni}}{\Longleftrightarrow} 	
			\forall x(x\in X\ \Longrightarrow\ \forall y[y\in Y\ \Longrightarrow\  P(x,y)])\\ 
			&\overset{(\text{no dependency})}{\Longleftrightarrow} 
			\forall x,\forall y\ (x\in X\ \Longrightarrow\ [y\in Y\ \Longrightarrow\ P(x,y)])\\ 
			&\overset{\ref{lemma:quant_laws},\ref{i:quant_scope_set}}{\Longleftrightarrow} 
			\forall y, \forall x\ (x\in X\ \Longrightarrow\ [y\in Y\ \Longrightarrow\ P(x,y)])\\ 
			&\overset{\ref{def:uni}}{\Longleftrightarrow} 
			\forall y,\ \forall x\in X\ (y\in Y\ \Longrightarrow\ P(x,y))\\ 
			&\overset{(\text{no dependency})}{\Longleftrightarrow} 
			\forall y\ (y\in Y\ \Longrightarrow\ \forall x\in X.\ P(x,y))\\ 
			&\overset{\ref{def:uni}}{\Longleftrightarrow} 
			\forall y\in Y,\ \forall x\in X.\ P(x,y)
		\end{align*}
		\item The following sequence holds:
		\begin{align*}
			\exists x\in X,\ \forall y\in Y.\  Q(x,y) &\overset{\ref{def:ex}}{\Longleftrightarrow} 	
			\exists x(x\in X\ \wedge\ \forall y\in Y.\  Q(x,y))\\ 
			&\overset{\ref{def:uni}}{\Longleftrightarrow} 
			\exists x(x\in X\ \wedge\ \forall y[y\in Y\ \Longrightarrow\ Q(x,y)])\\ 
			&\overset{(\text{no dependency})}{\Longleftrightarrow} 
			\exists x,\ \forall y(x\in X\ \wedge\ [y\in Y\ \Longrightarrow\ Q(x,y)])\\ 
			&\overset{\ref{lemma:quant_laws},\ref{i:quant}}{\Longrightarrow} 
			\forall y,\ \exists x(x\in X\ \wedge\ [y\in Y\ \Longrightarrow\ Q(x,y)])\\ 
			&\overset{\ref{def:ex}}{\Longleftrightarrow} 
			\forall y,\ \exists x\in X\ (y\in Y\ \Longrightarrow\ Q(x,y))\\ 
			&\overset{(\text{no dependency})}{\Longleftrightarrow} 
			\forall y\ (y\in Y\ \Longrightarrow\ \exists x\in X.Q(x,y))\\ 
			&\overset{\ref{def:uni}}{\Longleftrightarrow} 
			\forall y\in Y,\ \exists x\in X.Q(x,y)
		\end{align*}
		\item The following sequence holds:
		\begin{align*}
			\forall x\in X.\ P(x) \ \wedge\ \forall x\in X.\ Q(x) &\overset{\ref{def:uni}}{\Longleftrightarrow} 	
			\forall x(x\in X\ \Longrightarrow\ P(x))\ \wedge\ \forall x(x\in X\ \Longrightarrow\  Q(x))\\ 
			&\overset{\ref{lemma:quant_laws},\ref{i:forall_exists_set}}{\Longleftrightarrow} 
		\forall x[(x\in X\ \Longrightarrow\ P(x))\ \wedge\ (x\in X\ \Longrightarrow\  Q(x))]\\ 
%		&\Longleftrightarrow
%		\forall x[(x\not\in X\ \vee\ P(x))\ \wedge\ (x\not\in X\ \vee\  Q(x))]\\
%		&\overset{\text{Distributivity}}{\Longleftrightarrow} 
%		\forall x[x\not\in X\ \vee\ (P(x)\ \wedge\ Q(x))]\\
		& \Longleftrightarrow
		 \forall x[x\in X\ \Longrightarrow\ (P(x)\ \wedge\ Q(x))]\\
			&\overset{\ref{def:uni}}{\Longleftrightarrow} 
			\forall x\in X\ (P(x)\ \wedge\ Q(x))
		\end{align*}
		%
		\item
		The following sequence holds:
		\begin{align*}
			\forall x\in X.\ P(x) \ \vee\ \forall x\in X.\ Q(x) &\overset{\ref{def:uni}}{\Longleftrightarrow} 	
			\forall x(x\in X\ \Longrightarrow\ P(x))\ \vee\ \forall x(x\in X\ \Longrightarrow\  Q(x))\\ 
			&\overset{\ref{lemma:quant_laws},\ref{i:forall_set}}{\Longrightarrow} 
			\forall x[(x\in X\ \Longrightarrow\ P(x))\ \vee\ (x\in X\ \Longrightarrow\  Q(x))]\\ 
			& \Longleftrightarrow
			\forall x[x\in X\ \Longrightarrow\ (P(x)\ \vee\ Q(x))]\\
			&\overset{\ref{def:uni}}{\Longleftrightarrow} 
			\forall x\in X\ (P(x)\ \vee\ Q(x))
		\end{align*}
	\end{enumerate}
\end{proof}

%\begin{lemma}
%	\label{lemma:xz}
%	Let $b$ be a Boolean variable, $b\in\{0,1\}$. Let $x$ be an integer variable such that lower and upper bounds are known constants, $x_{lb}\leq x\leq x_{ub}$. Then the expression 
%	$y=b\cdot x$ can be written as a set of mixed-integer linear (MIL) constraints, i.e:
%	\begin{equation}
%		y=x\cdot b \quad \Longleftrightarrow\quad
%		\begin{aligned}
%			x_{lb}b\leq\  &y\leq x_{ub} b \\
%			x - x_{ub}(1-b) \leq &y \leq x- x_{lb}(1-b).
%		\end{aligned}
%	\end{equation}
%\end{lemma}
%\begin{proof}
%	First, note that since $b$ is Boolean, expression $y=x\cdot b$ is equivalent to:
%	\begin{equation}
%		\label{eq:T}
%		y = 
%		\begin{cases}
%			0,&\text{ if }b=0\\
%			x,&\text{ if }b=1.
%		\end{cases}
%	\end{equation}
%	
%	\begin{itemize}
%		\item$\Longrightarrow$ Let $y=x\cdot b$, therefore, \eqref{eq:T} holds. Substitution of these two cases ($b=0$ and $b=1$) into the inequalities lead to:
%		\begin{itemize}
%			\item $b=0$, $y=0$:
%			\begin{equation}
%				\begin{aligned}
%					0 \leq &0\leq 0\\
%					x-x_{ub} \leq &0 \leq x-x_{lb},\ \text{which means } x\leq x_{ub}\text{ and  }x\geq x_{lb} \text{ which holds due to the boundness of $x$.}
%				\end{aligned}
%			\end{equation}
%			Therefore, set of inequalities holds.
%			\item If $b=1$, $y=x$:
%			\begin{equation}
%				\begin{aligned}
%					x_{lb} \leq &x\leq x_{ub},\ \text{which holds due to the boundness of $x$.}\\
%					x\leq &x \leq x
%				\end{aligned}
%			\end{equation}
%		\end{itemize}
%		Therefore, set of inequalities hold. This completes proof of one way.
%		\item$\Longleftarrow$ Let the set of inequalities hold. Let us prove that $y=x\cdot b$. Since $b$ is Boolean consider two cases:
%		\begin{itemize}
%			\item $b=0$. Then from inequalities we get:
%			\begin{equation}
%				\begin{aligned}
%					0 \leq &y\leq 0\\
%					x-x_{ub} \leq &y \leq x-x_{lb}
%				\end{aligned}
%			\end{equation}
%			From first inequality we get that $y=0$, therefore, second inequality leads to $x\geq x_{lb}$ and $x\leq x_{ub}$ which hold. We showed that $b=0$ leads to $y=0$ and therefore, $y=x\cdot b$.
%			\item $b=1$.
%			\begin{equation}
%				\begin{aligned}
%					x_{lb} \leq &y\leq x_{ub}\\
%					x\leq &y \leq x
%				\end{aligned}
%			\end{equation}
%			Second inequality leads to $y=x$ and the first one gives the boundedness of $x$. Thus, we showed that $y=x\cdot b$. 
%		\end{itemize}
%	\end{itemize}
%\end{proof}
%
%\begin{rem}
%	Let $A$ and $B$ be integer values. Expression $C = \max(A,B)$ can be represented as a set of linear constraints as following:
%	\begin{align*}
%		C &\geq A\\
%		C &\geq B \\
%		C &\leq A+Mb \\
%		C &\leq B+M(1-b)
%	\end{align*}
%	where $b=\{0,1\}$ is an auxiliary binary variable and $M$ is a big-$M$ parameter ($M$ should be at least an upper bound on both $|A-B|$).
%\end{rem}
%Since $\min(A,B) = -\max(-A,-B)$ the $\min$ operator can be formulated as following:
%\begin{rem}
%	Let $A$ and $B$ be integer values. Expression $C = \min(A,B)$ can be represented as a set of linear constraints as following:
%	\begin{align*}
%		C &\leq A\\
%		C &\leq B \\
%		C &\geq A-Mb \\
%		C &\geq B-M(1-b)
%	\end{align*}
%	where $b=\{0,1\}$ is an auxiliary binary variable and $M$ is a big-$M$ parameter.
%\end{rem}
%A more general formulation is as follows:
%\begin{rem}
%	Expression $C = \min(a_1,\ldots,a_n)$ for $a_i\in\mathbb{R}$ can be represented as a set of linear constrains as following
%	\begin{align*}
%		C\leq a_i,\quad i=\{1,\ldots,n\}\\
%		C\geq a_i - M(1-b_i), \quad i=\{1,\ldots,n\}\\
%		\sum_{i=\{1,\ldots,n\}} b_i = 1
%	\end{align*}
%	where $b_i\in\{0,1\}$ is a binary variable that indicates the maximum $a_i$, and $M$ is a big-$M$ parameter. 
%\end{rem}
%\begin{rem}
%	Expression $C = \max(a_1,\ldots,a_n)$ for $a_i\in\mathbb{R}$ can be represented as a set of linear constrains as following
%	\begin{align*}
%		C\geq a_i,\quad i=\{1,\ldots,n\}\\
%		C\leq a_i + M(1-b_i), \quad i=\{1,\ldots,n\}\\
%		\sum_{i=\{1,\ldots,n\}} b_i = 1
%	\end{align*}
%	where $b_i\in\{0,1\}$ is a binary variable that indicates the maximum $a_i$, and $M$ is a big-$M$ parameter. 
%\end{rem}

==> chapters/proof_chi_sync.tex <==
\subsection{Proof of Theorem \ref{thm:chi_sync}}
$|\eta^{\pm}_\varphi(\sstraj,t)| \overset{\text{Def.}~\ref{def:time_rob_all}}{=} 
\sup\{\tau\geq0\, :\, \forall t'\in t \pm [0,\tau),\, \chi_\varphi(\sstraj,t')=\chi_\varphi(\sstraj,t)\}\!=\!\sup \varUpsilon\!=i>0$, 


If $i=+\infty$ the set is unbounded, so $\forall \tau\geq 0$ the $\chi$ property holds, i.e. $\forall t'\in t\pm[0,+\infty)$.

If $i<+\infty$ the set is bounded and we can apply the $\epsilon$ definition of supremum: 
$\forall \epsilon>0$, $\exists \tau^*\in \varUpsilon$ such that $\tau^*> i-\epsilon$.
i.e. the following holds:
\begin{equation}
	\label{eq:eps0}
	\forall \epsilon>0,\ \exists \tau^*\geq 0,\ \tau^*>i-\epsilon\ 
	\text{such that}\  \forall t'\in t\pm [0,\tau^*),\  \chi_\varphi(\sstraj,t')=\chi_\varphi(\sstraj,t).
\end{equation} 
Since $[0,i-\epsilon)\subseteq[0,\tau^*)$ then it holds that
\begin{equation}
	\label{eq:eps1}
	\forall \epsilon>0,\ \forall t'\in t\pm [0,i-\epsilon),\  \chi_\varphi(\sstraj,t')=\chi_\varphi(\sstraj,t).
\end{equation} 
%Now take any $t^*\in t\pm [0,i)$. We want to prove that $\chi_\varphi(\sstraj,t^*)=\chi_\varphi(\sstraj,t)$ holds.
%Since $t^*\in t\pm [0,i)$, there exists $\epsilon=\epsilon^*>0$ such that $t^*=t \pm (i - \epsilon^*)$. Now take another $\epsilon= \frac{\epsilon^*}{2}>0$ then due to \eqref{eq:eps1}, 
%$\forall t'\in t\pm \left[0,i-\frac{\epsilon^*}{2}\right)$,  $\chi_\varphi(\sstraj,t')=\chi_\varphi(\sstraj,t)$.
%Since $i-\epsilon^* \in [0,i-\frac{\epsilon^*}{2})$, then 
%for $t'=t \pm (i-\epsilon^*)$, $\chi_\varphi(\sstraj,t')=\chi_\varphi(\sstraj,t)$, thus, 
%$\chi_\varphi(\sstraj,t^*)=\chi_\varphi(\sstraj,t)$.
Assume the opposite of what is required to prove, i.e. assume that $\exists h\in [0, i)$ such that $\chi_\varphi(\sstraj,t\pm h)\not= \chi_\varphi(\sstraj,t)$. 
We can represent such $h$ as $h=i-\epsilon^*$ for some
$\epsilon^*$, $0<\epsilon^*\leq i$.
If we take $\epsilon=\frac{\epsilon^*}{2} >0$ then due to \eqref{eq:eps1},  
$\forall t'\in t\pm [0,i-\frac{\epsilon^*}{2})$, $\chi_\varphi(\sstraj,t')=\chi_\varphi(\sstraj,t)$.
Since $h=i-\epsilon^*\in [0, i-\frac{\epsilon^*}{2})$ then we know that
$\chi_\varphi(\sstraj,t\pm h)=\chi_\varphi(\sstraj,t)$ which contradicts with the above $\chi_\varphi(\sstraj,t\pm h)\not= \chi_\varphi(\sstraj,t)$.

==> chapters/proof_eta_neg.tex <==
\subsection{Proof of Remark \ref{rem:eta_neg}}
\begin{align*}
	\eta^{\pm}_{\neg\varphi}(\sstraj,t) &\overset{\text{Def.}\ref{def:time_rob_all}}{=} \chi_{\neg\varphi}(\sstraj, t)\cdot
	\sup\{\tau\geq0 \ :\ \forall t'\in[0,\tau],\ \chi_{\neg\varphi}(\sstraj,t \pm t')=\chi_{\neg\varphi}(\sstraj,t)\}\\
	&\overset{\text{Def.}\ref{def:char_func}}{=}
	-\chi_{\varphi}(\sstraj, t)\cdot
	\sup\{\tau\geq0 \ :\ \forall t'\in[0,\tau],\ \chi_{\varphi}(\sstraj,t \pm t')=\chi_{\varphi}(\sstraj,t)\}\\
	&\overset{\text{Def.}\ref{def:time_rob_all}}{=} -\eta^{\pm}_\varphi(\sstraj,t).
\end{align*}

==> chapters/proof_shift_async_sync.tex <==
\subsection{Quite Trivial Remark}

\begin{rem}
	Let $\varphi$ be an STL formula built upon the predicate set $AP$ and $\sstraj:\TDom \rightarrow X$ be a signal. For any time $t\in\TDom$ and $h\in\Re_{\geq 0}$, it holds that:
	\begin{equation}
		h < |\theta^{\pm}_\varphi(\sstraj,t)| \quad\Longrightarrow\quad 
		\chi_\varphi(\sstraj^{\leftrightarrows h},t )=\chi_\varphi(\sstraj,t).	
	\end{equation}
	\end{rem}

\begin{proof}
There exists two different proofs.
\begin{enumerate}
	\item 
	By Thm.~\ref{thm:shift_async} it holds that if $\max(h_1,\ldots,h_L) < |\theta^{\pm}_\varphi(\sstraj,t)|$ then $\chi_\varphi(\sstraj^{\leftrightarrows \bar{h}},t )=\chi_\varphi(\sstraj,t)$. Let $h_1=\ldots=h_L=h$, then it follows that if $h< |\theta^{\pm}_\varphi(\sstraj,t)|$ then 
	$\chi_\varphi(\sstraj^{\leftrightarrows \bar{h}},t )=\chi_\varphi(\sstraj,t)$. Since $\bar{h}=(h,\ldots,h)$ then trivially, $\sstraj^{\leftrightarrows \bar{h}}=\sstraj^{\leftrightarrows h}$ and thus, $\chi_\varphi(\sstraj^{\leftrightarrows h},t )=\chi_\varphi(\sstraj,t)$.	
	
	\item 
	
We are given that $h < |\theta^{\pm}_\varphi(\sstraj,t)|$. Then due to Thm.~\ref{thm:theta_bounded}, $h<|\theta^{\pm}_\varphi(\sstraj,t)|\leq |\eta^{\pm}_\varphi(\sstraj,t)|$. 
	Thus, by Thm.~\ref{thm:shift_sync_stronger}, $\chi_\varphi(\sstraj^{\leftrightarrows h},t )=\chi_\varphi(\sstraj,t)$.	
\end{enumerate}
	
\end{proof}


==> chapters/shift_async.tex <==
%\newpage
\subsection{Asynchronous Time Robustness}

\begin{definition}[Set of asynchronous shifts]
	\label{def:set_async}
	Let $\sstraj\in\SigSpace$ be a system trajectory, $AP=\{p_1,\ldots,p_L\}$ be a given set of predicates and $h_1,\ldots,h_L\in\Re_{\geq 0}$.
	The set of all trajectories $\mathbf{s}$ 
	that correspond to the
	asynchronous $h_1,\ldots,h_L$-early start APT
	is called a \textbf{set of asynchronous $\bm{h_1,\ldots,h_L}$ shifts to the left} \footnote{\color{red}maybe better to call this set a \textbf{set of asynchronous $h_1,\ldots,h_L$-early start trajectories}}, denoted as $\QI^{\leftarrow h_1,\ldots,h_L}(\sstraj)$, 
	i.e. 
	\begin{equation}
		\label{eq:QI}
		\QI^{\leftarrow h_1,\ldots,h_L}(\sstraj):=\left\{\mathbf{s}\in\SigSpace\ :
		\ 
		\bm{\chi}_\text{AP}^{}(\mathbf{s})=
		\APAL{h_1,\ldots,h_L}
		\right\}.
	\end{equation} 
	The \textbf{set of asynchronous $\bm{h_1,\ldots,h_L}$ shifts to the right} is defined analogously as:
	\begin{equation}
		\label{eq:QIR}
		\QI^{\rightarrow h_1,\ldots,h_L}(\sstraj):=\left\{\mathbf{s}\in\SigSpace\ :
		\ 
		\bm{\chi}_\text{AP}^{}(\mathbf{s})=
		\APAR{h_1,\ldots,h_L}
		\right\}.
	\end{equation} 
\end{definition}
Note that $\QI^{\leftrightarrows h_1,\ldots,h_L}(\sstraj)=\QA^{\leftrightarrows h}(\sstraj)$ if $h_1=\ldots=h_L=h$.


\begin{theorem}
	\label{thm:shift_async}
	For an STL formula $\varphi$ built upon the predicate set $AP$, trajectory $\sstraj:\TDom \rightarrow X$, time $t\in\TDom$ and some value $i\in\Re_{\geq 0}$, the following result holds:
	\begin{align*}
		|\theta^{\pm}_{\varphi}(\sstraj, t)|=i  \quad\Longrightarrow\quad
		&\forall h_1,\ldots,h_L\in[0, i),\ \forall \mathbf{s}\in\QI^{\leftrightarrows h_1,\ldots,h_L}(\sstraj),\quad 
		\chi_\varphi(\mathbf{s},t )=\chi_\varphi(\sstraj, t)
%		\\\Longrightarrow\quad
%		&\forall h\in [0, i),\ \forall\mathbf{s}\in \QA^{\leftrightarrows h}(\sstraj),\ \  \chi_\varphi(\mathbf{s}, t )=\chi_\varphi(\sstraj, t )	
	\end{align*}
\end{theorem}
A trivial consequence of Thm.~\ref{thm:shift_async} is formulated in the following remark. 
\begin{rem}
	\label{rem:shift_async_sync}
	For an STL formula $\varphi$ built upon the predicate set $AP$, trajectory $\sstraj:\TDom \rightarrow X$, time $t\in\TDom$ and some value $i\in\Re_{\geq 0}$, the following result holds:
	\begin{equation*}
		|\theta^{\pm}_{\varphi}(\sstraj, t)|=i  \quad\Longrightarrow\quad
		\forall h\in [0, i),\ \forall\mathbf{s}\in \QA^{\leftrightarrows h}(\sstraj),\ \  \chi_\varphi(\mathbf{s}, t )=\chi_\varphi(\sstraj, t )	
	\end{equation*}
\end{rem}



==> chapters/shift_sync.tex <==
\subsection{Synchronous Time Robustness}

\begin{definition}[Set of synchronous shifts]
	\label{def:set_sync}
	Let $\sstraj\in\SigSpace$ be a system trajectory, $AP$ be a given set of predicates and $h\in\Re_{\geq 0}$.
	The set of all trajectories $\mathbf{s}$ 
	that correspond to the
	synchronous $h$-early start APT
	is called a \textbf{set of synchronous $\bm{h}$ shifts to the left} \footnote{\color{red}maybe better to call this set a \textbf{set of synchronous $h$-early start trajectories}}, denoted as $\QA^{\leftarrow h}(\sstraj)$, 
	%($\QA^{\rightarrow h}(\sstraj)$), 
	i.e. 
	\begin{equation}
		\label{eq:QA}
		\QA^{\leftarrow h}(\sstraj):=\left\{\mathbf{s}\in\SigSpace\ :
		\ 
		\bm{\chi}_\text{AP}^{}(\mathbf{s})=
		\APSL{h}
		\right\}.
	\end{equation} 
The \textbf{set of synchronous $\bm{h}$ shifts to the right} is defined analogously as:
\begin{equation}
	\label{eq:QAR}
	\QA^{\rightarrow h}(\sstraj):=\left\{\mathbf{s}\in\SigSpace\ :
	\ 
	\bm{\chi}_\text{AP}^{}(\mathbf{s})=
	\APSR{h}
	\right\}.
\end{equation} 
\end{definition}
For example, trajectory
$\sstraj^{\leftarrow h}$ such that $\mathbf{x}^{\leftarrow h}(t)=\mathbf{x}(t+h)$, $\forall t\in\TDom$ 
belongs to the set of synchronous $h$ shifts to the left, 
$\sstraj^{\leftarrow h} \in\QA^{\leftarrow h}(\sstraj)$.
%and trajectory $\sstraj^{\rightarrow h}\in\QA^{\rightarrow h}(\sstraj)$. 
But  $\QA^{\leftarrow h}(\sstraj)$ is not limited to only $\sstraj^{\leftarrow h}$. In fact, it might contain infinite number of trajectories, since they can vary in shape in $X$. As long as the equality \eqref{eq:QA} holds on the APT level, such trajectories belong to $\QA^{\leftarrow h}(\sstraj)$. 

\begin{lemma}
	\label{lemma:sync_h}
	For an STL formula $\varphi$ built upon the predicate set $AP$,
	some $h\in\Re_{\geq 0}$ and two trajectories $\sstraj,\mathbf{s}:\TDom \rightarrow X$, 
\begin{equation*}
	\forall p\in AP,\ \bm{\chi}_p(\mathbf{s})=\bm{\chi}_p^{\leftrightarrows h}(\sstraj)	
	\quad\Longrightarrow\quad  \bm{\chi}_\varphi(\mathbf{s})=\bm{\chi}_\varphi^{\leftrightarrows h}(\sstraj).	
\end{equation*}
%	i.e. the function trajectory $\bm{\chi}_\varphi(\mathbf{s})$ of a synchronously shifted trajectory to the left (right) is a shifted to the left (right) function trajectory of the initial trajectory $\sstraj$.
	i.e. if trajectory $\mathbf{s}$ is a synchronously shifted trajectory $\sstraj$ to the left (right) by $h$, then the overall formula trajectory  $\bm{\chi}_\varphi(\mathbf{s})$ is going to be a shifted to the left (right) by $h$ formula trajectory $\bm{\chi}_\varphi(\sstraj)$. 
%	
%	If all predicate trajectories are synchronously shifted by $h$ then the overall formula trajectory will also be shifted by $h$. 
	\end{lemma}
	Using Def.~\ref{def:sync_asyn},\ref{def:sync_asyn_late} and \ref{def:set_sync}, the above result can equivalently be formulated as
\begin{equation*}
	\mathbf{s}\in\QA^{\leftrightarrows h}(\sstraj)\quad\Longrightarrow\quad 
	\forall t\in\TDom,\ \chi_\varphi(\mathbf{s},t )=\chi_\varphi(\sstraj, t\pm h).	
\end{equation*}

Note that only the implication holds for the above Lemma~\ref{lemma:sync_h}, i.e. there exist trajectories $\mathbf{s}\not\in\QA^{\leftrightarrows h}(\sstraj)$ for which $\bm{\chi}_\varphi(\mathbf{s})=\bm{\chi}_\varphi^{\leftrightarrows h}(\sstraj)$. For example, Fig.\ref{fig:phi_shift}(a) shows the characteristic function evaluation for predicates $p$, $q$ and formula $p\vee q$ for trajectory $\sstraj$. Fig.\ref{fig:phi_shift}(b) shows the same functions but for trajectory $\mathbf{s}$. One can see that though $\chi_{p\vee q}(\mathbf{s})=\chi^{\leftarrow 1}_{p\vee q}(\sstraj)$, its predicate trajectories are $\chi_{p}(\mathbf{s})=\chi^{\leftarrow 0}_{p}(\sstraj)$ and $\chi_{q}(\mathbf{s})=\chi^{\leftarrow 2}_{q}(\sstraj)$, therefore, $\mathbf{s}\not\in\QA^{\leftarrow 1}(\sstraj)$.

 
\begin{figure}[t!]
	\centering
		\includegraphics[width=\textwidth]{figures/phi_shift.pdf}
	\caption{Early and late start trajectories}
	\label{fig:phi_shift}
\end{figure}


\begin{theorem}
	\label{thm:shift_sync}
	For an STL formula $\varphi$ built upon the predicate set $AP$, trajectory $\sstraj:\TDom \rightarrow X$, time $t\in\TDom$ and some value $i\in\Re_{\geq 0}$, the following result holds:\footnote{
		{\color{red}
			I think it is possible to prove this stronger statement:
			\begin{align*}
				|\etap_\varphi(\sstraj, t)|=i\quad\Longleftrightarrow\quad
				&\forall h\in[0,i),\ \forall\mathbf{s}\in \QA^{\leftarrow h}(\sstraj),\ \  
				\chi_\varphi(\mathbf{s}, t )=\chi_\varphi(\sstraj, t ) \qquad\text{and}\\
				[&
				\forall\epsilon>0,\ \exists h\in[i, i+\epsilon),\ 
				\forall\mathbf{s}\in \QA^{\leftarrow h}(\sstraj),\ \  
				\chi_\varphi(\mathbf{s}, t )\not=\chi_\varphi(\sstraj, t )
				\quad\text{or}\quad 
				%	&\chi_{\varphi}(\sstraj,t \pm i)\not=\chi_\varphi(\sstraj,t)\quad \vee\\ 
				i=+\infty
				].
			\end{align*}
	}} 
	\begin{equation}
	\label{eq:shift_sync0}
	|\eta^{\pm}_\varphi(\sstraj,t)|=i \quad\Longrightarrow\quad
	\forall h\in[0, i),\ 
	\forall \mathbf{s}\in\QA^{\leftrightarrows h}(\sstraj)\quad 
	\chi_\varphi(\mathbf{s},t )=\chi_\varphi(\sstraj,t).	
\end{equation}
%\begin{equation}
%	|\eta^{\pm}_\varphi(\sstraj,t)|=i \quad\Longrightarrow\quad
%	\forall \mathbf{s}\in \bigcup_{h\in[0, i)}\QA^{\leftrightarrows h}(\sstraj)\quad 
%	\chi_\varphi(\mathbf{s},t )=\chi_\varphi(\sstraj,t).	
%\end{equation}
\end{theorem}



	
	












==> chapters/shifts.tex <==
\section{Properties of Time Robustness with Respect to Trajectory Shifts}
\label{sec:shifts}

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=\textwidth]{figures/sync_asyn(1).pdf}
%	\caption{Early start trajectories: (a) shows a specific AP trajectory that consists of three predicate trajectories of time horizon $H$, (b) depicts a synchronous $h$-early start trajectory and (c) draws an asynchronous $h_1,h_2,h_3$-early start trajectory.}
%	\label{fig:sync_asyn}
%	\vspace{-5mm}
%\end{figure}
%
%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=\textwidth]{figures/sync_asyn(2).pdf}
%	\caption{Early start trajectories: (a) shows a specific AP trajectory that consists of three predicate trajectories of time horizon $H$, (b) depicts a synchronous $h$-early start trajectory and (c) draws an asynchronous $h_1,h_2,h_3$-early start trajectory.}
%	\label{fig:sync_asyn}
%	\vspace{-5mm}
%\end{figure}


\begin{figure}[t!]
	\centering
	\begin{subfigure}[b]{\textwidth}
	\includegraphics[width=\textwidth]{figures/shifts.pdf}
	\caption{Early start trajectories: (a) shows a specific APT that consists of three PTs, (b) depicts a synchronous $h$-early start APT and (c) draws an asynchronous $h_1,h_2,h_3$-early start APT.}
	\label{fig:sync_asyn}
	\end{subfigure}
	
	\begin{subfigure}[b]{\textwidth}
	\includegraphics[width=\textwidth]{figures/shifts_async.pdf}
	\caption{Late start trajectories: (a) shows a specific APT that consists of three PTs, (b) depicts a synchronous $h$-late start APT and (c) draws an asynchronous $h_1,h_2,h_3$-late start APT.}
	\label{fig:sync_asyn2}
	\end{subfigure}
	\caption{Early and late start trajectories}
	\label{fig:shifts}
\end{figure}


\begin{definition}
	Let $\sstraj\in\SigSpace$ be a system trajectory.
	\begin{itemize}
		\item For a given predicate $p\in AP$ we call $\bm\chi_{p}(\sstraj):\SigSpace \to \{\pm 1\}^{\TDom}$ (an image of $\sstraj$ through the characteristic function $\chi_{p}$) a \textbf{predicate trajectory (PT)}.
		\item For a given formula $\varphi$ we call $\bm\chi_{\varphi}(\sstraj):\SigSpace \to \{\pm 1\}^{\TDom}$ (an image of $\sstraj$ through the characteristic function $\chi_{\varphi}$) a \textbf{formula trajectory (FT)}.
		\item For a given set of predicates $AP=\{p_1,\ldots,p_L\}$ a concatenation of all predicate trajectories 
		$\bm{\chi}_\text{AP}^{}(\mathbf{x})=
		\begin{bmatrix}
			\bm{\chi}_{p_1}(\mathbf{x})\\
			\vdots\\
			\bm{\chi}_{p_L}(\mathbf{x})
		\end{bmatrix}\in \{\pm 1\}^{L \times \TDom}$ defines an \textbf{AP-trajectory (APT)}.
	\end{itemize}
	
\end{definition}

	
	
%{\color{blue}
%\begin{exmp}
%		Take a look at Fig.~\ref{fig:shifts}, describe Fig.~\ref{fig:sync_asyn} and Fig.~\ref{fig:sync_asyn2}.
%		Explain informally the idea of shifts. Add that in red one can see that traj parts that are ignored, in transparent blue - extended random values that do not change SAT of $\varphi$. Then read the following formal Def~\ref{def:sync_asyn}.
%\end{exmp}
%}

\begin{definition}[Early start]
	\label{def:sync_asyn}
		Let $\bm{\chi}_p(\sstraj)$ be a PT and 
		$\bm{\chi}_\text{AP}^{}(\mathbf{x})$ be an APT for a given system trajectory $\sstraj$, predicate $p$ and a set $AP=\{p_1,\ldots,p_L\}$. For a given $h, h_1,\ldots,h_L\in\Re_{\geq 0}$, 
		\begin{itemize}
			\item $\bm{h}$\textbf{-early start PT}, denoted $\bm{\chi}^{\leftarrow h}_p(\sstraj)$, is a PT that is shifted by $h$ to the left: 
			\begin{equation}
			\chi^{\leftarrow h}_p(\sstraj,t)=\chi_p(\sstraj,t+h),\ \forall t\in\TDom
			\end{equation}
			where $\chi^{\leftarrow h}_p(\sstraj,t)$ is the $t$-th element of $\bm{\chi}^{\leftarrow h}_p(\sstraj)$.
			%
			\item \textbf{Synchronous} $\bm{h}$\textbf{-early start APT}, denoted $\APSL{h}$, is an APT with all its PTs being $h$-early start PTs, i.e. all PTs are synchronously shifted by $h$  to the left: 
			\begin{equation}
				\APSL{h}=
				\begin{bmatrix}
					\bm{\chi}_{p_1}^{\leftarrow h}(\mathbf{x})\\
					\vdots\\
					\bm{\chi}_{p_L}^{\leftarrow h}(\mathbf{x})
				\end{bmatrix}
				%\in {\{\pm1\} }^{L\times(H-h+1)}	
			\end{equation}
			%
			\item \textbf{Asynchronous} $\bm{h_1},\ldots,\bm{h_L}$\textbf{-early start APT}, denoted $\APAL{h_1,\ldots,h_L}$, is an APT with each $i$-th PT being a $h_i$-early start PT,
			i.e. PTs are asynchronously shifted to the left, each by its own number: 
			\begin{equation}
				\APAL{h_1,\ldots,h_L}=
				\begin{bmatrix}
					\bm{\chi}_{p_1}^{\leftarrow h_1}(\mathbf{x})\\
					\vdots\\
					\bm{\chi}_{p_L}^{\leftarrow h_L}(\mathbf{x})
				\end{bmatrix}
				%\in {\{\pm1\} }^{L\times(H-h+1)}	
			\end{equation} 
		\end{itemize}
	\end{definition}
%Note that when $h_1=\ldots=h_L=h$, $\bm{\chi}^{\leftarrow h_1,\ldots,h_L}_{\text{AP, asyn}}(\sstraj)=\APSL{h}$.

\begin{definition}[Late start]
	\label{def:sync_asyn_late}
The late start trajectories  $\bm{\chi}^{\rightarrow h}_p(\sstraj)$, $\APSR{h}$ and $\APAR{h_1,\ldots,h_L}$ can be defined analogously to Def.~\ref{def:sync_asyn} but with shifts to the right, see Fig.~\ref{fig:sync_asyn2}. 
\end{definition}








==> chapters/shifts_x.tex <==
%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=\textwidth]{figures/early_traj.pdf}
%	\caption{Early start signals.  (a) Predicate signals $\bm\chi_{p_1}(\sstraj)$, $\bm\chi_{p_2}(\sstraj)$ and $\bm\chi_{p_3}(\sstraj)$ of a specific signal  $\sstraj$; (b) a synchronous $h$-early start trajectory $\sstraj^{\leftarrow h}$; (c) an asynchronous $\bar{h}$-early start trajectory $\sstraj^{\leftarrow \bar{h}}$, where $\bar{h}=(h_1, h_2, h_3)$.}
%	\label{fig:early_traj}
%\end{figure}

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=\textwidth]{figures/early_signal.pdf}
%	\caption{Early signals. (a) Signal $\sstraj=[\sstraj_{(1)},\, \sstraj_{(2)}]^\top$; (b) predicate signals $\bm\chi_{p_1}(\sstraj)$, $\bm\chi_{p_2}(\sstraj)$ and $\bm\chi_{p_3}(\sstraj)$ of signal  $\sstraj$; (c) predicate signals $\bm{\chi}_{p_i}(\sstraj^{\leftarrow h})$ which equal to the synchronously shifted by $h$ predicate signals $\bm{\chi}_{p_i}(\sstraj)$, $i=\{1,2,3\}$, i.e. \eqref{eq:synch_shift} holds; (d) predicate signals $\bm{\chi}_{p_i}(\sstraj^{\leftarrow \bar{h}})$, $\bar{h}=(h_1, h_2, h_3)$ which are equal to the asynchronously shifted by $h_i$ predicate signals $\bm{\chi}_{p_i}(\sstraj)$, $i=\{1,2,3\}$, i.e. \eqref{eq:asynch_shift} holds.}
%	\label{fig:early_traj}
%\end{figure}


	
	




	

	
	
%{\color{blue}
%\begin{exmp}
%		Take a look at Fig.~\ref{fig:shifts}, describe Fig.~\ref{fig:sync_asyn} and Fig.~\ref{fig:sync_asyn2}.
%		Explain informally the idea of shifts. Add that in red one can see that traj parts that are ignored, in transparent blue - extended random values that do not change SAT of $\varphi$. Then read the following formal Def~\ref{def:sync_asyn}.
%\end{exmp}
%}

%\begin{definition}[Early and late start PT]
%	\label{def:sync_asyn}
%		Let $\bm{\chi}_p(\sstraj)$ be a PT for a given system trajectory $\sstraj$ and a predicate $p$. For a given $h\in\Re_{\geq 0}$, 
%		\begin{itemize}
%			\item $\bm{h}$\textbf{-early start PT}, denoted $\bm{\chi}^{\leftarrow h}_p(\sstraj)$, is a PT that is shifted by $h$ to the left: 
%			\begin{equation}
%			\chi^{\leftarrow h}_p(\sstraj,t)=\chi_p(\sstraj,t+h),\ \forall t\in\TDom
%			\end{equation}
%			%
%			\item $\bm{h}$\textbf{-late start PT}, denoted $\bm{\chi}^{\rightarrow h}_p(\sstraj)$, is a PT that is shifted by $h$ to the right: 
%			\begin{equation}
%				\chi^{\rightarrow h}_p(\sstraj,t)=\chi_p(\sstraj,t-h),\ \forall t\in\TDom
%			\end{equation}
%			where $\chi^{\leftarrow h}_p(\sstraj,t)$ is the $t$-th element of $\bm{\chi}^{\leftarrow h}_p(\sstraj)$.
%		\end{itemize}
%	\end{definition}
%Note that when $h_1=\ldots=h_L=h$, $\bm{\chi}^{\leftarrow h_1,\ldots,h_L}_{\text{AP, asyn}}(\sstraj)=\APSL{h}$.

%see Fig.~\ref{fig:sync_asyn2}.









==> chapters/test_circuit.tex <==
\subsection{The RC Oscillator Circuit}

In a Resistance-Capacitance Oscillator or simply known as an RC Oscillator, we can make use of the fact that a phase shift occurs between the input to a RC network and the output from the same network by using interconnected RC elements in the feedback branch, for example:
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.7\textwidth]{figures/rc_osc.jpg}
	\caption{PICTURE FROM INTERNET.}
	\label{fig:rc_osc}
\end{figure}

 The amount of actual phase shift in the circuit depends upon the values of the resistor (R) and the capacitor (C), at the chosen frequency of oscillations with the phase angle ($\varphi$). 

Plan is: 
\begin{itemize}
	\item Write down a meaningful specification $\varphi$ that combines input and output signals from the given circuit.
	\item For a given circuit solve the control-synthesis problem and find max time robustness together with default signals.
	\item Knowing $\theta$ we know we can shift output signal `by as much' therefore, we can modify the circuit elements up to this given bound.
\end{itemize}

==> chapters/test_truck.tex <==
\subsection{Truck delivery problem (Traveling salesman problem)}




\begin{figure}[h!]
	\centering
	\includegraphics[width=.9\textwidth]{figures/truck_map.png}
	\caption{Goods delivery map.}
	\label{fig:truck_map}
\end{figure}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.95\textwidth]{figures/truck_eta.pdf}
	\caption{Truck trajectory generated by solving
		Problem~\ref{prob:synthesis} with objective $\objs\defeq \etap_{\varphi_{\text{truck}}}$. Found maximum right synchronous time robustness is 
		$\etap_{\varphi_{\text{truck}}}(\trajsync,0) = 12$ hours. Driver is performing goods pickup and delivery in specific locations.
		Initial position is marked by $\star$.}
	\label{fig:truck_eta}
\end{figure}



In this case study we are interested in the optimal trajectory planning for a truck driver, who needs to pick up and deliver goods across the US. The driver starts from Kansas City and his destination list consists of Chicago, Columbus and Philadelphia, in a specific order, specified by the following STL specification:
\begin{align*}
	\varphi_{\text{truck}}\defeq
	\eventually_{[10, 15]}\always_{[0,\, 4]} &(x\in\text{Chicago})\  \wedge\\
	&\eventually_{[25, 30]}\always_{[0,\, 4]} \left(x\in\text{Columbus}\right)
	\wedge\eventually_{[45, 50]} \left(x\in\text{Philly}\right). 
\end{align*}
with $x_0 \in \text{Kansas City}$. Variable $x$ denotes the truck position in the two dimensional space. In more details, starting from Kansas City, the truck driver should reach Chicago any time between $10$ and $15$ hours and stay there for 4 hours required for goods loading. Next he must arrive to Columbus anytime between $25$ and $30$ hours and stay there again for 4 hours straight. Finally, the driver must reach Philadelphia and finish the delivery route anywhere from $45$ to $50$ hours (floating destination time).

The loading time might include gas refills, pick up, drop off and break times for the driver. Due to various uncertainties and a long horizon of the mission, the higher values of the temporal robustness are preferred. For instance, maximization of the right synchronous time robustness $\etap_\varphi(\sstraj,0)$ would allow driver to have the freedom in starting the execution of the found trajectory earlier (therefore, arriving to all locations earlier), while still satisfying the mission specification. On the other hand, maximization of the right asynchronous time robustness $\thetap_\varphi(\sstraj,0)$, gives the driver the freedom in arriving to individual destinations earlier (each by different amount of time), while still satisfying the specification. Therefore, the temporal robustness maximization approach on top of Boolean satisfaction increases the truck driver comfort and freedom.


For simulations, we set the discrete-time trajectory horizon to be $H\defeq 70$, we refer to time units as hours. 
In order to generate an optimal trajectory, we solved the time-robust control synthesis problem~\ref{prob:synthesis} two times: once with the right synchronous temporal robustness objective $\objs\defeq \etap_{\varphi_{\text{truck}}}$ and once with the right asynchronous temporal robustness $\objs\defeq \thetap_{\varphi_{\text{truck}}}$.

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.95\textwidth]{figures/truck_theta.pdf}
	\caption{Truck trajectory generated by solving
		Problem~\ref{prob:synthesis} with objective $\objs\defeq \thetap_{\varphi_{\text{truck}}}$. Found maximum right asynchronous time robustness is 
		$\thetap_{\varphi_{\text{truck}}}(\trajasyn,0) = 10$ hours. Driver is performing goods pickup and delivery in specific locations.
		Initial position is marked by $\star$.}
	\label{fig:truck_theta}
\end{figure}

Found maximum synchronous right time robustness is $\etap_{\varphi_{\text{truck}}}(\trajsync,0) = 12$ hours, see Fig.~\ref{fig:truck_eta}.
One can see that the generated trajectory $\trajsync$ satisfies the mission specification, i.e., $\chi_{\varphi_{\text{truck}}}(\trajsync,0)=1$. On top of that the driver is allowed to start the trajectory execution by up to $12$ hours earlier and still succeed in mission completion. This is so since $\etap_{\varphi_{\text{truck}}}(\trajsync,0) = 12$, and thus, due to Thm.~\ref{thm:shift_sync_stronger_disc}, $\forall h\in [0, 12]$, $\chi_{\varphi_{\text{truck}}}(\trajsync^{\leftarrow h},0)=1$. This is easily seen in Fig.~\ref{fig:truck_eta}(b), where $\forall t'\in t+ [0, 12]$, $\chi_{\varphi}(\sstraj,t')=1$ and 
$\chi_{\varphi}(\sstraj,t +13)=-1$, which means that the right side of Thm.~\ref{thm:chi_sync_stronger_disc} is satisfied. One can also see, that if we shift independent predicates in time asynchronously, see Fig.~\ref{fig:truck_eta}(c),(d) and (e), meaning the truck driver will arrive to Chicago earlier by $h_1$, earlier to Columbus by $h_2$ and earlier to Philly by $h_3$, even if $\max(h_1,h_2,h_3)\leq 12$, the specification $\varphi_{\text{truck}}$ will be violated for such asynchronous $\bar{h}$-early trajectory.

%Total yalmiptime time is $0.6$ second and solver time is 2.54 seconds.
%178 continuous, 1262 integer variables.
		
Found maximum asynchronous right time robustness is $\thetap_{\varphi_{\text{truck}}}(\trajasyn,0) = 10$ hours, see Fig.~\ref{fig:truck_theta}.
In this case, we are allowed to shift predicates asynchronously by up to $10$ hours and the mission will still be satisfied, see Fig.~\ref{fig:truck_theta}(c),(d) and (e).
%Total yalmiptime time is 1 second and solver time is 153 seconds.
%	2164 continuous, 2361 integer variables.




